Parallel Global Edge Switching for the Uniform Sampling of Simple Graphs with Prescribed Degrees

The uniform sampling of simple graphs matching a prescribed degree sequence is an important tool in network science, e.g. to construct graph generators or null-models. Here, the Edge Switching Markov Chain (ES-MC) is a common choice. Given an arbitrary simple graph with the required degree sequence, ES-MC carries out a large number of small changes, called edge switches, to eventually obtain a uniform sample. In practice, reasonably short runs efficiently yield approximate uniform samples. In this work, we study the problem of executing edge switches in parallel. We discuss parallelizations of ES-MC, but find that this approach suffers from complex dependencies between edge switches. For this reason, we propose the Global Edge Switching Markov Chain (G-ES-MC), an ES-MC variant with simpler dependencies. We show that G-ES-MC converges to the uniform distribution and design shared-memory parallel algorithms for ES-MC and G-ES-MC. In an empirical evaluation, we provide evidence that G-ES-MC requires not more switches than ES-MC (and often fewer), and demonstrate the efficiency and scalability of our parallel G-ES-MC implementation.

==> eager-algorithms.tex <==
\pares is a simplistic parallelization of \esmc to establish a performance baseline for parallel algorithms.
Each PU (processing unit) performs switches independently while synchronizing implicitly only by preventing concurrent updates of individual edges.
To ensure that no edge is erased or inserted twice, we store the edges in a concurrent hash-set using the following semantics:
to remove an edge from the set, a ticket has to be acquired first; this can be done by locking an existing edge or by inserting-and-locking a new edge.
These operations are implemented using a compare-and-exchange primitive.
Concurrent updates to the same edge are sequenced by the hardware.

To perform an edge switch, a PU draws the indices of two edges $i, j \in [m]$ (independently of other PUs) and then attempts to rewire the edges $E[i]$ and $E[j]$ as in \cref{def:ses}.
To this end, it first attempts to lock the two source edges and then to insert-and-lock the target edges.
If any of them is already locked by a concurrent edge switch, the PU releases all locks it might hold to prevent dead locks, and then restarts using the same edge indices (observe that $E[i]$ and $E[j]$ might be different after the restart).
If any of the target edges exists and is unlocked, the switch is rejected as ordinary.
%An implementation of \pares is shown in Algorithm \ref{algo:eageres}.

We call this algorithm \emph{eager}, as it performs every edge switch that is legal after synchronization, but lacks a well-defined order.
Instead, the order in which edge switches are performed is left up to the scheduler\footnote{On real hardware, a combination of the CPU, memory subsystem, and OS.}.
This however can lead to deviations from the intended Markov Chain.
For example, consider two edge switches that are performed in parallel, and are legal, but attempt to insert the same edge, causing a target dependency.
In that case, only the edge switch whose PU is able to lock both its target edges first is successful, and the other switch fails.
Therefore, the transition probability between two adjacent states in the state graph, is not only determined by the probability of selecting the two source edges, but also by the probability of the switch having a target dependency and the probability of being scheduled first.

Even in the case of a fair scheduler that grants each edge switch the same probability of being scheduled first, the probability of the switch having a target dependency is not symmetric between adjacent states.
For example, consider two adjacent states $A \ne B$, where $A$ contains the edges $\{u, v\}, \{a, b\}$ and $B$ contains the edges $\{u, a\}, \{v, b\}$.
The probability that an edge switch between $A$ and $B$ encounters a target dependency is equal to the probability that another switch attempts to insert either one of the same edges.
However, for the edge switch $A \to B$, the probability that another switch attempts to insert either $\{u, a\}$ or $\{v, b\}$ is proportional to the node degrees $\deg(u) \deg(a) + \deg(v) \deg(b)$, whereas for the edge switch  $B \to A$, the probability is proportional to $\deg(u) \deg(v) + \deg(a) \deg(b)$.

In conclusion, while this algorithm is simple to describe and implement, it does not faithfully implement \esmc.
To do so, we need to take into account the dependencies between the switches and ensure that switches with dependencies are processed in a well-defined order.
%As discussed in \cref{sec:g-es-mc}, this is more difficult for \esmc as it exhibits both source and target dependencies.
%In particular, if an edge switch has a source dependency on another, then the target edges of the second switch can only be determined once we know whether the first switch is legal.
%Thus, source dependencies make it difficult to even detect other dependencies deeper into the dependency chain.

%We might consider an algorithm that performs edge switches in batches, and choose a small enough batch size so that each batch contains only target dependencies with high probability.
%This requires the batch size to be very small, e.g. at most $O(\sqrt{m})$ switches.
%However, this algorithm is unlikely to scale well, as we may only parallelize small batches of $O(\sqrt{m})$ switches each, but must perform $\Omega(\sqrt{m})$ batches sequentially to even perform $m$ switches in total.
%\gesmc on the other hand, does not exhibit source dependencies by design, and allows us to parallelize global switches of up to $\lfloor m / 2 \rfloor$ single edge switches each.

%\begin{myalgorithm}[t]
%	\KwData{edge list $E$ of a simple graph, requested switches $r$}
%	
%	\tcp{Initialize edge hash set $H$}
%	Let $H \gets \emptyset$\;
%	\ParFor{each edge $e \in E$}{
%		H.insert($e$)\;
%	}
%	
%	\ParFor{$i$ from $1$ to $r$}{
%		\tcp{Independently sample an edge switch $\sigma$}
%		Sample edge indices $i, j \sim [m]$ with $i \neq j$\;
%		Sample direction bit $g \sim \{0, 1\}$\;
%		\tcp{Lock the source edges}
%		Let $t_1, t_2$ be tickets for the source edges\;
%		\While{not both $t_1, t_2$ acquired}{
%			Let $e_1 = E[i]$\;
%			$t_1 \gets H.$lock($e_1$)\;
%			\If{$t_1$ acquired}{
%				Let $e_2 = E[j]$\;
%				$t_2 \gets H.$lock($e_2$)\;
%				\If{not $t_2$ acquired}{
%					$H$.release($e_1, t_1$)
%				}
%			}
%		}
%		Compute target edges $(\vec e_3, \vec e_4) = \tau(\vec e_1, \vec e_2, g)$\;
%		\tcp{Lock the target edges}
%		Let $t_3, t_4$ be tickets for the target edges\;
%		\While{not both $t_3, t_4$ acquired}{
%			$t_3 \gets H.$lock($e_3$)\;
%			\If{$t_3$ acquired}{
%				$t_4 \gets H.$lock($e_4$)\;
%				\If{not $t_4$ acquired}{
%					$H$.release($e_3, t_3$)\;
%				}
%			}
%		}	
%		\If{$e_3$ is not self-loop $\land$ $e_4$ is not self-loop}{
%			\If{$H$.insert($e_3, t_3$) succeeds}{
%				\If{$H$.insert($e_4, t_4$) succeeds}{
%					%\tcp{Success, rewire the edges}
%					$E[i] \gets e_3, E[j] \gets e_4$\;
%					$\forall i \in \{1, 2\}\colon$\ $H$.erase($e_i, t_i$)\;
%				}
%				\Else{
%					$H$.erase($e_3, t_3$)\;
%				}
%			}
%			$\forall i \in \{3, 4\}\colon$\ $H$.release($e_i, t_i$)\;
%		}
%		$\forall i \in \{1, 2\}\colon$\ $H$.release($e_i, t_i$)\;
%	}
	
%	\caption{\pares}
%	\label{algo:eageres}
%\end{myalgorithm}
